Multi-Perspective Data Augmentation for Few-shot Object Detection

Recent few-shot object detection (FSOD) methods have focused on augmenting synthetic samples for novel classes, show promising results to the rise of diffusion models. However, the diversity of such datasets is often limited in representativeness because they lack awareness of typical and hard samples, especially in the context of foreground and background relationships. To tackle this issue, we propose a Multi-Perspective Data Augmentation (MPAD) framework. In terms of foreground-foreground relationships, we propose in-context learning for object synthesis (ICOS) with bounding box adjustments to enhance the detail and spatial information of synthetic samples. Inspired by the large margin principle, support samples play a vital role in defining class boundaries. Therefore, we design a Harmonic Prompt Aggregation Scheduler (HPAS) to mix prompt embeddings at each time step of the generation process in diffusion models, producing hard novel samples. For foreground-background relationships, we introduce a Background Proposal method (BAP) to sample typical and hard backgrounds. Extensive experiments on multiple FSOD benchmarks demonstrate the effectiveness of our approach. Our framework significantly outperforms traditional methods, achieving an average increase of $17.5\%$ in nAP50 over the baseline on PASCAL VOC. Code is available at https://github.com/nvakhoa/MPAD.

==> 2_related_work.tex <==
\section{Related work}
\label{sec:related_word}
FSOD methods~\cite{meta-rcnn, yolo-reweighting, rpn-attention, TFA, max-margin, trans-int, meta-detr, han2022few, bulat2023fs} are designed to identify and classify novel objects with limited data. With two learning strategies: Meta-learning-based FSOD methods, ~\cite{meta-rcnn} and ~\cite{yolo-reweighting} generating distinct features by adjusting the weights of query and support features. ~\cite{max-margin, trans-int, rpn-attention, hu2021dense, meta-detr, han2022few, bulat2023fs} enhance feature representation through various techniques, including max-margin optimization, data augmentation; Transfer learning-based FSOD approaches~\cite{TFA, defrcn, guirguis2023niff, zhu2021semantic, li2023disentangle,vu2023instance, xu2023generating} focus on efficiently leveraging foundational knowledge. TFA~\cite{TFA} freezes most network layers during the fine-tuning phase, DeFRCN~\cite{defrcn} introduces gates to modulate gradients across modules. ~\cite{vu2023instance} utilizes hierarchical information by employing augmentation strategies through language models for feature enhancement.
 

With limited data samples in computer vision tasks, a branch of approaches tends to synthesize additional data by utilizing generative models. Some approaches \cite{li2023gligen, zhuang2023task} have demonstrated the ability to generate images with a provided prior structure via bounding boxes, masks, etc. Power-Paint \cite{zhuang2023task}, with its context-aware image inpainting, enables the regeneration of new objects while maintaining context and background in the identified region via a bounding box. ~\cite{lin2023explore, fang2024data} utilize the power of synthesis data by diffusion model and adapter module for FSOD problems. ~\cite{lin2023explore} combine a copy-paste pipeline and Stable Diffusion \cite{rombach2022high} in the data generation process. The new novel instances were selected and pasted in the random backgrounds from the base class sets. \cite{fang2024data} integrate ControlNet to generate visual priors and CLIP Rank for filtering synthetic samples. However, these methods do not comprehensively exploit aspects of data augmentation. To the best of our knowledge, our method is the first to thoroughly explore the primary aspects of data synthesis.
